ExPrIS: Knowledge-Level Expectations as Priors for Object Interpretation from Sensor Data

While deep learning has significantly advanced robotic object recognition, purely data-driven approaches often lack semantic consistency and fail to leverage valuable, pre-existing knowledge about the environment. This report presents the ExPrIS project, which addresses this challenge by investigating how knowledge-level expectations can serve as to improve object interpretation from sensor data. Our approach is based on the incremental construction of a 3D Semantic Scene Graph (3DSSG). We integrate expectations from two sources: contextual priors from past observations and semantic knowledge from external graphs like ConceptNet. These are embedded into a heterogeneous Graph Neural Network (GNN) to create an expectation-biased inference process. This method moves beyond static, frame-by-frame analysis to enhance the robustness and consistency of scene understanding over time. The report details this architecture, its evaluation, and outlines its planned integration on a mobile robotic platform.

==> ki2025_project_report_expris_architecture.tex <==
%\documentclass[tikz, border=10pt]{standalone}
%\usepackage[utf8]{inputenc}
%\usepackage[T1]{fontenc}
%\usepackage{helvet} 
%
%\usetikzlibrary{shapes.geometric, arrows.meta, positioning, fit, backgrounds, calc, shapes.misc}
%
%\renewcommand{\familydefault}{\sfdefault}

% Farben
%\definecolor{exbg}{RGB}{235, 248, 235}    
%\definecolor{exnode}{RGB}{180, 235, 180}  
%\definecolor{mapblue}{RGB}{160, 215, 255} 
%\definecolor{liebg}{RGB}{253, 250, 235}   
%\definecolor{lienode}{RGB}{255, 245, 200} 

%\begin{document}

\begin{tikzpicture}[
    base/.style={
        rectangle, 
        rounded corners=15pt, 
        draw=black!90, 
        thick, 
        align=center, 
        font=\small\sffamily
    },
    green_node/.style={
        base, 
        fill=exnode, 
        % Feste Breite erzwingen, damit beide unteren Boxen gleich sind
        text width=3.5cm, 
        minimum height=2cm
    },
    blue_node/.style={
        base, 
        fill=mapblue, 
        text width=4cm, 
        minimum height=3.6cm,
        rounded corners=10pt
    },
    yellow_node/.style={
        base, 
        fill=lienode, 
        draw=gray!80,
        text=gray!90,
        % selbe Breite wie untere green nodes
        text width=3.5cm,
        minimum height=2cm
    },
    line/.style={
        draw=black!80, 
        thick, 
        -{Stealth[length=3mm, width=2mm]}
    },
    label_text/.style={
        font=\footnotesize\sffamily, 
        align=center, 
        text=black!80
    }
]

    % --- 1. Hauptachse (Horizontal) ---
    % Wir platzieren Map, GNN und VLM alle auf y=0 (anchor=center).
    % Das garantiert, dass der Pfeil VLM -> Map horizontal ist.

    % Mitte
    \node[blue_node] (map) at (0,0) {\textbf{3DSSG Semantic Map}\\(Dynamic Environment\\Representation)\\(Sec.~\ref{sec:semantic-mapping-with-3dssgs})};

    % Links (GNN) - Abstand zur Map definiert
    \node[green_node, left=3cm of map, minimum width=4.5cm, text width=4.5cm] (gnn) {Expectation-Biased GNN\\Prediction (Sec.~\ref{sec:expectation-biased-ml})};

    % Rechts (VLM) - Abstand zur Map definiert
    \node[yellow_node, right=3cm of map, minimum width=4.5cm, text width=4.5cm] (vlm) {Vision-Language Models\\(e.g., CLIP)};


    % --- 2. Untere Ebene (Links) ---
    % Wir positionieren die unteren Boxen relativ zum GNN, aber symmetrisch.
    
    % Sensor Data (verschoben nach links unten)
    \node[green_node] (sensor) at ($(gnn.south) + (-2.2, -2.5)$) {Sensor Data (Single RGB-D\\Frame)};

    % External Knowledge (verschoben nach rechts unten)
    \node[green_node] (ext_know) at ($(gnn.south) + (2.2, -2.5)$) {External Knowledge Graph\\(e.g., ConceptNet)};


    % --- 3. Untere Ebene (Rechts) ---
    % Reasoning (verschoben nach links unten)
    \node[yellow_node] (reasoning) at ($(vlm.south) + (-2.2, -2.5)$) {Open-Vocabulary Reasoning};

    % Query (verschoben nach rechts unten)
    \node[yellow_node] (query) at ($(vlm.south) + (2.2, -2.5)$) {Natural Language Query\\(``Find the dishwasher'')};

    % --- 4. Verbindungen ---

    % Sensor -> GNN (Pfeilspitze unten links)
    \draw[line] (sensor.north) -- ([xshift=-0.4cm]gnn.south);

    % Ext Know -> GNN (Pfeilspitze unten rechts) + Label
    \draw[line] (ext_know.north) -- ([xshift=0.4cm]gnn.south) node[midway, fill=exbg, inner sep=2pt, label_text] {Semantic Knowledge};

    % GNN <-> Map (Parallel)
    % Update Graph (oben)
    \draw[line] ([yshift=0.4cm]gnn.east) -- ([yshift=0.4cm]map.west) node[midway, above, label_text] {update graph};
    % Contextual Priors (unten)
    \draw[line] ([yshift=-0.4cm]map.west) -- ([yshift=-0.4cm]gnn.east) node[midway, below, label_text] {contextual priors\\(from observation\\history)};

    % Query -> Reasoning
    \draw[line, draw=gray] (query.west) -- (reasoning.east);

    % Map -> Reasoning
    \draw[line, draw=gray] ([yshift=-0.4cm]map.east) -- (reasoning.north) node[midway, fill=liebg, inner sep=2pt, label_text, text=gray!90] {features \& structure};

    % VLM -> Map
    \draw[line, draw=gray] ([yshift=0.4cm]vlm.west) -- ([yshift=0.4cm]map.east) node[midway, below, label_text, text=gray!90] {vision-language\\features};


    % --- 5. Hintergründe (Perfekt ausgerichtet) ---
    
    % Wir berechnen globale Grenzen für oben und unten, damit beide Container gleich hoch sind.
    % Oben: Gleich wie Map
    % Unten: Ein Stück unter Sensor/Query
    \coordinate (top_limit) at (map.north);
    \coordinate (bot_limit) at ($(sensor.south)!0.5!(query.south) - (0, 0.6)$);

    \begin{scope}[on background layer]
        
        % --- ExPrIS Container ---
        \path let \p1=(top_limit), \p2=(bot_limit), 
                  \p3=(sensor.west), \p4=(map.west) in 
              node[
                draw=black!80, thick, fill=exbg, rounded corners=20pt,
                inner sep=0pt, % Wir steuern den Platz manuell
                fit={(\x3-0.5cm, \y1) (\x4-0.5cm, \y2)} 
              ] (expris_bg) {};

        \node[anchor=north west, font=\Large\sffamily, text=black] at (expris_bg.north west) [xshift=0.5cm, yshift=-0.5cm] {ExPrIS};

        % --- LIEREx Container ---
        \path let \p1=(top_limit), \p2=(bot_limit), 
                  \p3=(map.east), \p4=(query.east) in 
              node[
                draw=gray!80, dashed, thick, fill=liebg, rounded corners=20pt,
                inner sep=0pt,
                fit={(\x3+0.5cm, \y1) (\x4+0.5cm, \y2)}
              ] (lierex_bg) {};
              
        \node[anchor=north west, font=\Large\sffamily, text=gray] at (lierex_bg.north west) [xshift=0.5cm, yshift=-0.5cm] {LIEREx};

    \end{scope}

\end{tikzpicture}
%\end{document}

